A Practical, Progressively-Expressive GNN

Message passing neural networks (MPNNs) have become a dominant flavor of graph neural networks (GNNs) in recent years. Yet, MPNNs come with notable limitations; namely, they are at most as powerful as the 1-dimensional Weisfeiler-Leman (1-WL) test in distinguishing graphs in a graph isomorphism testing frame-work. To this end, researchers have drawn inspiration from the k-WL hierarchy to develop more expressive GNNs. However, current k-WL-equivalent GNNs are not practical for even small values of k, as k-WL becomes combinatorially more complex as k grows. At the same time, several works have found great empirical success in graph learning tasks without highly expressive models, implying that chasing expressiveness with a coarse-grained ruler of expressivity like k-WL is often unneeded in practical tasks. To truly understand the expressiveness-complexity tradeoff, one desires a more fine-grained ruler, which can more gradually increase expressiveness. Our work puts forth such a proposal: Namely, we first propose the (k, c)(<=)-SETWL hierarchy with greatly reduced complexity from k-WL, achieved by moving from k-tuples of nodes to sets with <=k nodes defined over <=c connected components in the induced original graph. We show favorable theoretical results for this model in relation to k-WL, and concretize it via (k, c)(<=)-SETGNN, which is as expressive as (k, c)(<=)-SETWL. Our model is practical and progressively-expressive, increasing in power with k and c. We demonstrate effectiveness on several benchmark datasets, achieving several state-of-the-art results with runtime and memory usage applicable to practical graphs. We open source our implementation at https://github.com/LingxiaoShawn/KCSetGNN.

==> 99-Checklist.tex <==

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}{}
  \item Did you describe the limitations of your work?
    \answerNo{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{In Appendix}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Will add later into the URL}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In Appendix}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In Appendix}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> TABLE/qm9.tex <==



%\begin{table}[]
\begin{wraptable}{r}{6.3cm}
\caption{\method performances on QM9  by varying ($k$,$c$). Test MAE at lowest Val. MAE highlighted in \textbf{bold}.
All variances are lower than 0.002 and omitted. GINE with 4 and 6 layers shown as baseline.}
    \label{tab:qm9bykc}
	{\scalebox{0.8}{
\begin{tabular}{rrlll}
\toprule
 & &  {Train loss}      & {Val.} MAE         & {Test MAE}         \\\midrule
{$(k$} & {$c)$} & $\leq${\sc SetGNN}     &          &       \\
\midrule
2 & 1 & 0.0376               & 0.0387               & 0.0389               \\
3 & 1 & 0.0308               & 0.0386               & 0.0379               \\
4 & 1 & 0.0338               & 0.0371               & 0.0370               \\
5 & 1 & 0.0311               & 0.0345               & 0.0343               \\
6 & 1 & 0.0216               & 0.0299               & 0.0289               \\
7 & 1 & 0.0203               & {0.0282}               & {0.0272}               \\
\midrule
2 & 2 & 0.0363               & 0.0419               & 0.0394               \\
3 & 2 & 0.0276               & 0.0371               & 0.0359               \\
4 & 2 & 0.0229               & 0.0284               & 0.0269               \\
5 & 2     & 0.0175               & \textbf{0.0267}               & \textbf{0.0251}                     \\
\midrule
3 & 3 & 0.0294              & 0.0372              & 0.0373             \\
4 & 3 & 0.0208               & 0.0312               & 0.0282   \\
\hline \hline
\multicolumn{2}{l}{GINE} ($L$$=$$4$) &  0.0507 &	0.0478 &	0.0479 \\
\multicolumn{2}{l}{GINE} ($L$$=$$6$) & 0.0440 &	0.0440 &	0.0451 \\
\bottomrule
\end{tabular}
}}
\end{wraptable}



==> TABLE/zinc.tex <==


%\begin{table}[!ht]
\begin{wraptable}{r}{7.2cm}
\caption{\method performances on ZINC-12K  by varying ($k$,$c$). Test MAE at lowest Val. MAE highlighted in \textbf{bold}.}
    \label{tab:zincbykc}
	{\scalebox{0.8}{
\begin{tabular}{rrlll}
\toprule
\multicolumn{1}{l}{$k$} & \multicolumn{1}{l}{$c$} & {Train loss}      & {Val.} MAE         & {Test MAE}        \\
\midrule
2                     & 1                     & 0.1381 ± 0.0240 & 0.2429 ± 0.0071 & 0.2345 ± 0.0131 \\

3                     & 1                     & 0.1172 ± 0.0063 & 0.2298 ± 0.0060 & 0.2252 ± 0.0030 \\


4                     & 1                     & 0.0693 ± 0.0111 & 0.1645 ± 0.0052 & 0.1636 ± 0.0052 \\
5                     & 1                     & 0.0643 ± 0.0019 & 0.1593 ± 0.0051 & 0.1447 ± 0.0013 \\
6                     & 1                     & 0.0519 ± 0.0064 & 0.0994 ± 0.0093 & 0.0843 ± 0.0048 \\
7                     & 1                     & 0.0543 ± 0.0048 & 0.0965 ± 0.0061 & 0.0747 ± 0.0022 \\
8                     & 1                     & 0.0564 ± 0.0152 & 0.0961 ± 0.0043 & 0.0732 ± 0.0037 \\
9                     & 1                     & 0.0817 ± 0.0274 & 0.0909 ± 0.0094 & 0.0824 ± 0.0056 \\
10                    & 1                     & 0.0894 ± 0.0266 & 0.1060 ± 0.0157 & 0.0950 ± 0.0102 \\
\midrule
2                     & 2                     & 0.1783 ± 0.0602 & 0.2913 ± 0.0102 & 0.2948 ± 0.0210 \\
3                     & 2                     & 0.0640 ± 0.0072 & 0.1668 ± 0.0078 & 0.1391 ± 0.0102 \\
4                     & 2                     & 0.0499 ± 0.0043 & 0.1029 ± 0.0033 & 0.0836 ± 0.0010 \\
5                     & 2                     & 0.0483 ± 0.0017 & \textbf{0.0899 ± 0.0056} & \textbf{0.0750 ± 0.0027} \\
6                     & 2                     & 0.0530 ± 0.0064 & 0.0927 ± 0.0050 & 0.0737 ± 0.0006 \\
7                     & 2                     & 0.0547 ± 0.0036 & 0.0984 ± 0.0047 & 0.0784 ± 0.0043 \\
\midrule
3                     & 3                     & 0.0798 ± 0.0062 & 0.1881 ± 0.0076 & 0.1722 ± 0.0086 \\
4                     & 3                     & 0.0565 ± 0.0059 & 0.1121 ± 0.0066 & 0.0869 ± 0.0026 \\
5                     & 3                     & 0.0671 ± 0.0156 & 0.1091 ± 0.0097 & 0.0920 ± 0.0054 \\
\bottomrule
\end{tabular}
}}
\end{wraptable}
